Selecting the number of clusters, clustering models, and algorithms. A unifying approach based on the quadratic discriminant score

Cluster analysis requires many decisions: the clustering method and the implied reference model, the number of clusters and, often, several hyper-parameters and algorithms' tunings. In practice, one produces several partitions, and a final one is chosen based on validation or selection criteria. There exist an abundance of validation methods that, implicitly or explicitly, assume a certain clustering notion. Moreover, they are often restricted to operate on partitions obtained from a specific method. In this paper, we focus on groups that can be well separated by quadratic or linear boundaries. The reference cluster concept is defined through the quadratic discriminant score function and parameters describing clusters' size, center and scatter. We develop two cluster-quality criteria called quadratic scores. We show that these criteria are consistent with groups generated from a general class of elliptically-symmetric distributions. The quest for this type of groups is common in applications. The connection with likelihood theory for mixture models and model-based clustering is investigated. Based on bootstrap resampling of the quadratic scores, we propose a selection rule that allows choosing among many clustering solutions. The proposed method has the distinctive advantage that it can compare partitions that cannot be compared with other state-of-the-art methods. Extensive numerical experiments and the analysis of real data show that, even if some competing methods turn out to be superior in some setups, the proposed methodology achieves a better overall performance.

==> parts/custom.tex <==
\usepackage[english]{babel}
%\usepackage[hyphens]{url}
\usepackage{xr-hyper}
%\usepackage[pdftex = true, colorlinks=true, citecolor=blue, linkcolor=blue,urlcolor=blue, breaklinks=true, bookmarksnumbered=true, bookmarksopen=true, bookmarksopenlevel=1]{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{amsthm}
\usepackage{natbib}
\usepackage{xcolor}
\usepackage{color}
\usepackage{graphicx}
\usepackage{datetime}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{float}
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{soul}
% \usepackage{emptypage}
% \usepackage[font=small, labelfont=bf]{caption}
\usepackage{rotating}
\usepackage{subfig}
%% \usepackage[inline]{showlabels}
%\usepackage[ruled, vlined]{algorithm2e}
\usepackage{adjustbox}
\usepackage{multirow}



%% MISC
%% ---------------------------------------------
%% graphics format hierarchy
\DeclareGraphicsExtensions{.pdf,.png,.jpg,.jpeg}

%% notes highlight
\definecolor{colNOTE}{HTML}{ED2E38}
\newcommand{\NOTE}[1]{\textcolor{colNOTE}{/*~\textsf{#1}~*/\xspace}}

%% package names and functions
\newcommand{\pkg}[1]{\textsf{#1}\xspace}
\newcommand{\methodset}[1]{\MakeLowercase{\textsc{#1}}\xspace}

%% latin acronyms:  e.g. i.e. etc.
\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\vs}{vs.\@\xspace}
\makeatletter
\newcommand*{\etc}{%
\@ifnextchar{.}%
{etc}%
{etc.\@\xspace}%
}
\makeatother

%% acronym for cross-ref to supplementary materials
\newcommand{\mpf}{{\sc pf}}
\newcommand{\smf}{{\sc smf}}

%% Commands for supporting info
\newcommand{\sisec}[1]{SI Appendix, Section~S#1}
\newcommand{\sifig}[1]{SI Appendix, Figure~S#1}
\newcommand{\sitab}[1]{SI Appendix, Table~S#1}
\newcommand{\sialgo}[1]{SI Appendix, Algorithm~S#1}


%% ref to figures and tables
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\subsecref}[1]{Subsection~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}

%% ordinal numbers
\newcommand{\nst}{-\emph{st}\xspace}
\newcommand{\nnd}{-\emph{nd}\xspace}
\newcommand{\nrd}{-\emph{rd}\xspace}
\newcommand{\nth}{-\emph{th}\xspace}
% \newcommand{\nst}{{\raise0.5ex\hbox{\footnotesize{st}}}\xspace}
% \newcommand{\nnd}{{\raise0.5ex\hbox{\footnotesize{nd}}}\xspace}
% \newcommand{\nrd}{{\raise0.5ex\hbox{\footnotesize{rd}}}\xspace}
% \newcommand{\nth}{{\raise0.5ex\hbox{\footnotesize{th}}}\xspace}






%% Statements
%% ----------------------------------------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}




%% Math
%% ------------------------------------------------------
\newcommand{\eps}{\varepsilon}
\newcommand{\abs}[1]{\left| {#1} \right|}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\inner}[1]{\left\langle {#1} \right\rangle}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\indfun}[2]{\ind_{#1}{\left(#2\right)}}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\setR}{\mathbb{R}}
\newcommand{\setN}{\mathbb{N}}
\newcommand{\inv}[1]{{#1}^{\scriptsize -1}}
\newcommand{\tra}[1]{{#1}^\mathsf{T}}
\newcommand{\invtra}[1]{{#1}^\mathsf{T}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\maximize}{Maximize}
\DeclareMathOperator*{\minimize}{Minimize}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spec}{Spec}
\DeclareMathOperator{\vect}{vec}




%% Statistics and probability
%% -------------------------------------------------------------------------
%%\newcommand{\Prob}[1]{\Pr\!\left\{ #1 \right\}}%
\DeclareMathOperator{\oPr}{Pr}
\newcommand{\prob}[2][]{{\oPr_{#1}}{\left\{#2\right\}}}
\DeclareMathOperator{\oE}{E}
\newcommand{\E}[2][]{{\oE_{#1}}{\left[#2\right]}}
\DeclareMathOperator{\oVar}{Var}
\newcommand{\Var}[2][]{{\oVar_{#1}}{\left[#2\right]}}
\DeclareMathOperator{\oCov}{Cov}
\newcommand{\Cov}[2][]{{\oCov_{#1}}{\left[#2\right]}}
\DeclareMathOperator{\oCor}{Cor}
\newcommand{\Cor}[2][]{{\oCor_{#1}}{\left[#2\right]}}
\newcommand{\given}{\,{\,\vert\,}\,}
\newcommand{\givenn}{\,{\,\big\vert\,}\,}
\newcommand{\givennn}{\,{\,\Bigg\vert\,}\,}
\newcommand{\iidsim}{\,\overset{\text{iid}}{\scalebox{1.25}{$\sim$}}\,}
\newcommand{\convas}{\stackrel{\sf as}{\longrightarrow}}
\newcommand{\convp}{\stackrel{\sf p}{\longrightarrow}}
\newcommand{\convms}{\stackrel{\sf ms}{\longrightarrow}}
\newcommand{\convd}{\stackrel{\sf d}{\longrightarrow}}







%% Paper specific notation
%% -------------------------------------

%% tagging conditions
\newcommand{\cndGaussian}{{\normalfont (C1)}\xspace}
\newcommand{\cndEqualPrecision}{{\normalfont (C2)}\xspace}
\newcommand{\cndInfDiffLoglik}{{\normalfont (C3)}\xspace}


%% matrices
\newcommand{\bI}{\bm{I}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bA}{\bm{A}}


%% vectors
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bbeta}{\bm{\beta}}

%% sequences
\newcommand{\otn}{1,\allowbreak 2, \allowbreak \ldots, \allowbreak n}
\newcommand{\otK}{1,\allowbreak 2, \allowbreak \ldots, \allowbreak K}
\newcommand{\otM}{1,\allowbreak 2, \allowbreak \ldots, \allowbreak M}

%% operators
\DeclareMathOperator{\qs}{qs}
\DeclareMathOperator{\lik}{lik}
\DeclareMathOperator{\clik}{clik}
\DeclareMathOperator{\ent}{ent}
\DeclareMathOperator{\ec}{ec}
\DeclareMathOperator{\AIC}{AIC}
\DeclareMathOperator{\BIC}{BIC}
\DeclareMathOperator{\ICL}{ICL}
\DeclareMathOperator{\CH}{CH}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\ASW}{ASW}
\DeclareMathOperator{\dkl}{d_{KL}}

%% recurrent objects 
\newcommand{\bthetam}{\btheta^{(m)}}
\newcommand{\hbtheta}{\hat{\btheta}_{n}}
\newcommand{\hbthetam}{\hat{\btheta}^{(m)}_n}
\newcommand{\pim}{\pi^{(m)}}
\newcommand{\bmum}{\bmu^{(m)}}
\newcommand{\bSigmam}{\bSigma^{(m)}}
\newcommand{\Hd}{H(\cdot)}
\newcommand{\Td}{T(\cdot)}
\newcommand{\Hnd}{H_n(\cdot)}
\newcommand{\Tnd}{T_n(\cdot)}
\newcommand{\Fn}{\mathbb{F}_n}





==> tables/algorithm_x_criteria.tex <==
\begin{table}[!htpb]
   \centering
   \caption{Possibility to compute clustering quality criteria (columns) by clustering algorithms (rows).}\label{tab:algorithm_x_criteria}
   \scriptsize
   \begin{tabular}{lccccccccccccc}
       \toprule
       &AIC &BIC &ICL &ASW &CH &FW &CVLK &HS &SS &CVHS &CVSS &BTHS &BTSS \\
       \midrule
       K-means & & & &\checkmark &\checkmark &\checkmark & &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
       K-medoids & & & &\checkmark &\checkmark &\checkmark & &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
       Mclust &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
       Rimle & & & &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
       Emmix &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
       \bottomrule
   \end{tabular}
\end{table}


==> tables/auxiliary/banknote_1000b.tex <==
%latex.default(tab, numeric.dollar = FALSE, booktabs = TRUE, table.env = TRUE,     file = paste0("../../paper/tables/auxiliary/", dataset, ".tex"),     label = paste0("tab:", dataset), title = "Criterion", caption = "<++>")%
\begin{table}[!tbp]
\caption{<++>\label{tab:banknote_1000b}} 
\begin{center}
\begin{tabular}{lrllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
\midrule
BEST ARI& 2&Rimle&$\gamma$: $1$ pam&$1$&$0$\tabularnewline
BEST VIC& 2&Rimle&$\gamma$: $1$ pam&$1$&$0$\tabularnewline
AIC& 6&Emmix&mvt; ncov: 3&$0.6$&$-1.16$\tabularnewline
BIC& 3&Mclust& VVE&$0.84$&$-0.43$\tabularnewline
ICL& 3&Mclust& VVE&$0.84$&$-0.43$\tabularnewline
QH&10&Rimle&$\gamma$: $10000$ pam&$0.26$&$-2.14$\tabularnewline
QS&10&Rimle&$\gamma$: $10000$ pam&$0.26$&$-2.14$\tabularnewline
CH& 2&Rimle&$\gamma$: $1$ pam&$\mathbf{1}$&$\mathbf{0}$\tabularnewline
ASW& 2&Rimle&$\gamma$: $1$ kmeans&$\mathbf{1}$&$\mathbf{0}$\tabularnewline
FW& 2&Rimle&$\gamma$: $100$ kmeans&$0.98$&$-0.08$\tabularnewline
CVLK& 3&Rimle&$\gamma$: $10$ InitClust&$0.85$&$-0.42$\tabularnewline
CVQH& 3&Mclust& VEV&$0.78$&$-0.62$\tabularnewline
CVQS& 3&Mclust& VEV&$0.78$&$-0.62$\tabularnewline
BQH& 3&Rimle&$\gamma$: $10$ kmeans&$0.86$&$-0.37$\tabularnewline
BQS& 3&Rimle&$\gamma$: $10$ kmeans&$0.86$&$-0.37$\tabularnewline
\bottomrule
\end{tabular}\end{center}
\end{table}


==> tables/auxiliary/iris_1000b.tex <==
%latex.default(tab, numeric.dollar = FALSE, booktabs = TRUE, table.env = TRUE,     file = paste0("../../paper/tables/auxiliary/", dataset, ".tex"),     label = paste0("tab:", dataset), title = "Criterion", caption = "<++>")%
\begin{table}[!tbp]
\caption{<++>\label{tab:iris_1000b}} 
\begin{center}
\begin{tabular}{lrllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
\midrule
BEST ARI&3&Mclust& EEE&$0.94$&$-0.26$\tabularnewline
BEST VIC&3&Mclust& EEE&$0.94$&$-0.26$\tabularnewline
AIC&6&Emmix&mvt; ncov: 3&$0.57$&$-1.52$\tabularnewline
BIC&2&Mclust& VEV&$0.57$&$-0.67$\tabularnewline
ICL&2&Mclust& VEV&$0.57$&$-0.67$\tabularnewline
QH&7&Emmix&mvt; ncov: 4&$0.42$&$-1.56$\tabularnewline
QS&7&Emmix&mvt; ncov: 4&$0.42$&$-1.56$\tabularnewline
CH&3&Mclust& EII&$0.73$&$-0.76$\tabularnewline
ASW&2&Mclust& EVV&$0.57$&$-0.67$\tabularnewline
FW&2&Mclust& VII&$0.57$&$-0.67$\tabularnewline
CVLK&4&Rimle&$\gamma$: $10000$ InitClust&$0.81$&$-0.57$\tabularnewline
CVQH&4&Rimle&$\gamma$: $10000$ InitClust&$0.81$&$-0.57$\tabularnewline
CVQS&4&Rimle&$\gamma$: $1000$ InitClust&$0.81$&$-0.58$\tabularnewline
BQH&3&Rimle&$\gamma$: $100$ pam&$\mathbf{0.9}$&$\mathbf{-0.32}$\tabularnewline
BQS&3&Rimle&$\gamma$: $100$ pam&$\mathbf{0.9}$&$\mathbf{-0.32}$\tabularnewline
\bottomrule
\end{tabular}\end{center}
\end{table}


==> tables/auxiliary/olive_1000b_class1.tex <==
%latex.default(tab, numeric.dollar = FALSE, booktabs = TRUE, table.env = TRUE,     file = paste0("../../paper/tables/auxiliary/", dataset, ".tex"),     label = paste0("tab:", dataset), title = "Criterion", caption = "<++>")%
\begin{table}[!tbp]
\caption{<++>\label{tab:olive_1000b_class1}} 
\begin{center}
\begin{tabular}{lrllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
\midrule
BEST ARI& 3&Emmix&mvt; ncov: 3&$1$&$-0.03$\tabularnewline
BEST VIC& 3&Emmix&mvt; ncov: 3&$1$&$-0.03$\tabularnewline
AIC&10&Emmix&mvt; ncov: 3&$0.33$&$-1.74$\tabularnewline
BIC& 6&Emmix&mvt; ncov: 3&$0.52$&$-1.42$\tabularnewline
ICL& 6&Emmix&mvt; ncov: 3&$0.52$&$-1.42$\tabularnewline
QH&10&Mclust& VVV&$0.29$&$-1.84$\tabularnewline
QS&10&Mclust& VVV&$0.29$&$-1.84$\tabularnewline
CH& 3&K-Means&&$0.32$&$-1.88$\tabularnewline
ASW& 2&Emmix&mvt; ncov: 5&$0.39$&$-1.28$\tabularnewline
FW& 2&Emmix&mvt; ncov: 3&$\mathbf{0.82}$&$\mathbf{-0.42}$\tabularnewline
CVLK&10&Rimle&$\gamma$: $1000$ InitClust&$0.3$&$-1.81$\tabularnewline
CVQH& 7&Emmix&mvt; ncov: 3&$0.28$&$-2.04$\tabularnewline
CVQS& 7&Emmix&mvt; ncov: 3&$0.28$&$-2.04$\tabularnewline
BQH& 8&Mclust& VVV&$0.49$&$-1.28$\tabularnewline
BQS& 8&Mclust& VVV&$0.49$&$-1.28$\tabularnewline
\bottomrule
\end{tabular}\end{center}
\end{table}


==> tables/auxiliary/olive_1000b_class2.tex <==
%latex.default(tab, numeric.dollar = FALSE, booktabs = TRUE, table.env = TRUE,     file = paste0("../../paper/tables/auxiliary/", dataset, ".tex"),     label = paste0("tab:", dataset), title = "Criterion", caption = "<++>")%
\begin{table}[!tbp]
\caption{<++>\label{tab:olive_1000b_class2}} 
\begin{center}
\begin{tabular}{lrllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
\midrule
BEST ARI& 8&Mclust& EVE&$0.88$&$-0.65$\tabularnewline
BEST VIC& 8&Mclust& EVE&$0.88$&$-0.65$\tabularnewline
AIC&10&Emmix&mvt; ncov: 3&$0.47$&$-1.77$\tabularnewline
BIC& 6&Emmix&mvt; ncov: 3&$0.76$&$-1.32$\tabularnewline
ICL& 6&Emmix&mvt; ncov: 3&$0.76$&$-1.32$\tabularnewline
QH&10&Mclust& VVV&$0.54$&$-1.26$\tabularnewline
QS&10&Mclust& VVV&$0.54$&$-1.26$\tabularnewline
CH& 3&K-Means&&$0.42$&$-2.28$\tabularnewline
ASW& 2&Emmix&mvt; ncov: 5&$0.29$&$-2.28$\tabularnewline
FW& 2&Emmix&mvt; ncov: 3&$0.36$&$-1.84$\tabularnewline
CVLK&10&Rimle&$\gamma$: $1000$ InitClust&$0.58$&$-1.18$\tabularnewline
CVQH& 7&Emmix&mvt; ncov: 3&$0.44$&$-1.96$\tabularnewline
CVQS& 7&Emmix&mvt; ncov: 3&$0.44$&$-1.96$\tabularnewline
BQH& 8&Mclust& VVV&$\mathbf{0.86}$&$\mathbf{-0.74}$\tabularnewline
BQS& 8&Mclust& VVV&$\mathbf{0.86}$&$\mathbf{-0.74}$\tabularnewline
\bottomrule
\end{tabular}\end{center}
\end{table}


==> tables/clustering_models.tex <==
% Table for clustering models
\begin{table}[!tbp]
    \caption{Clustering models in the experimental analysis. The total number of models (``\#Models'') for each algorithm is obtained combining ``\#K'' and ``Other configurations''.}\label{tab:clustering_models}
    \scriptsize
    \centering
    \begin{tabularx}{\linewidth}{ l l r r X X }
        \toprule
        Algorithm &Clustering strategy &\#Models &\#K &Other configurations &Software\\
        \midrule
        K-means &Distance-based &10 &1-10 & &\cite{rcore2021r}\\
        K-medoids &Distance-based &10 &1-10 & &\cite{maechler2021cluster}\\
        Mclust &Gaussian mixtures & 140 &1-10 &14 Covariance parametrizations (\cite{celeux1995gaussian}) &\cite{mclust2016paper}\\
        Rimle &Gaussian mixtures & 180 &1-10 &$\gamma \in \set{1,5,10,100,1000,10000}$; 3 initialization methods. &\cite{coretto2016consistency, coretto2016robust, coretto2021otrimle}\\
        Emmix &t-student mixtures & 100 &1-10 &5 Covariance parametrizations; skewed and not-skewed t-distributions &\cite{wang2018emmixskew}\\
        \bottomrule
    \end{tabularx}
\end{table}


==> tables/data_designs.tex <==
% Table for simulated designs
\begin{table}[!tbp]
    \caption{Real data and simulated designs. Number of simulated points, dimensionality and true number of clusters are given as $n$, $d$ and $K$ respectively.}\label{tab:data_designs}
    \scriptsize
    \centering
    \begin{tabularx}{\linewidth}{ l r r r X }
        \toprule
        Data/Design &n &d &K &Short Description\\
        \midrule
        Iris &$150$ &$4$ &$3$ &Measurements on Iris flowers; two classes show substantial overlap.\\
        Banknote &$200$ &$6$ &$2$  &Measurements on original and counterfeit bills; the latter class is usually split in more groups due to the high variability of the measurements.\\
        Olive &$572$ &$8$ &$3$/$9$ &Measurements on olive oils' fatty acids, having two different classifications; some classes scatters are concentrated on lower dimensional hyperplanes and show substantial overlap. \\
        \midrule
        Pentagon5 &$300$ &$2$ &$5$ &Mixture of uneven Gaussian distributions; strong pairwise overlap of 4 of the 5 components.\\
        Uniform &$300$ &$2$ &$1$ &Two-dimensional uniform distribution; many criteria are not able to identify the unclustered case.\\
        Flower2 &$300$ &$2$ &$5$ &Mixture of 2 t-shaped, 2 uniform  and one spherical Gaussian components; features regions of strong cluster overlaps.\\
        T52D &$300$ &$2$ &$5$ &Mixture of 5 equal-proportions t-Student distributions.\\
        T510D &$300$ &$10$ &$5$ &Adds 8 unclustered dimensions to the T52D design to increase dimensionality without adding new clustering information.\\
        \bottomrule
    \end{tabularx}
\end{table}


==> tables/real_tables.tex <==
\begin{sidewaystable}
\tiny
\centering
\caption{Clustering solutions selected by the 13 selection criteria under comparison on the three real data sets. First two rows in each table indicate the two best feasible solutions: \textsc{best ari} and \textsc{best vic} partitions. The column ``K'' reports  the number of groups discovered by the selected solution. The ``Algorithm'' and ``Configuration'' columns identify the specific member of $\mathcal{M}$ that is selected. The nomenclature used in the previous columns is defined in Section~S5-(\smf). Finally, the ARI and the VIC columns measure the agreement of the selected partition with respect to the ground truth.
\label{tab:real_tables}}
    \subfloat[][Iris dataset]{
        \begin{tabular}{lrllrr}
        \toprule
        \multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
        \midrule
        BEST ARI&3&Mclust& EEE&$0.94$&$-0.26$\tabularnewline
        BEST VIC&3&Mclust& EEE&$0.94$&$-0.26$\tabularnewline
        \midrule
        AIC&6&Emmix&mvt; $\text{ncov}=3$&$0.57$&$-1.52$\tabularnewline
        BIC&2&Mclust& VEV&$0.57$&$-0.67$\tabularnewline
        ICL&2&Mclust& VEV&$0.57$&$-0.67$\tabularnewline
        QH&7&Emmix&mvt; $\text{ncov}=4$&$0.42$&$-1.56$\tabularnewline
        QS&7&Emmix&mvt; $\text{ncov}=4$&$0.42$&$-1.56$\tabularnewline
        CH&3&Mclust& EII&$0.73$&$-0.76$\tabularnewline
        ASW&2&Mclust& EVV&$0.57$&$-0.67$\tabularnewline
        FW&2&Mclust& VII&$0.57$&$-0.67$\tabularnewline
        CVLK&4&Rimle&$\gamma=10000$; InitClust&$0.81$&$-0.57$\tabularnewline
        CVQH&4&Rimle&$\gamma=10000$; InitClust&$0.81$&$-0.57$\tabularnewline
        CVQS&4&Rimle&$\gamma=1000$; InitClust&$0.81$&$-0.58$\tabularnewline
        BQH&3&Rimle&$\gamma=100$; pam&$\mathbf{0.9}$&$\mathbf{-0.32}$\tabularnewline
        BQS&3&Rimle&$\gamma=100$; pam&$\mathbf{0.9}$&$\mathbf{-0.32}$\tabularnewline
        \bottomrule
        \end{tabular}
    }
    \subfloat[][Banknote dataset]{
        \begin{tabular}{lrllrr}
        \toprule
        \multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
        \midrule
        BEST ARI& 2&Mclust& EII&$1$&$0$\tabularnewline
        BEST VIC& 2&Mclust& EII&$1$&$0$\tabularnewline
        \midrule
        AIC& 6&Emmix&mvt; $\text{ncov}=3$&$0.6$&$-1.16$\tabularnewline
        BIC& 3&Mclust& VVE&$0.84$&$-0.43$\tabularnewline
        ICL& 3&Mclust& VVE&$0.84$&$-0.43$\tabularnewline
        QH&10&Rimle&$\gamma=10000$; pam&$0.26$&$-2.14$\tabularnewline
        QS&10&Rimle&$\gamma=10000$; pam&$0.26$&$-2.14$\tabularnewline
        CH& 2&Rimle&$\gamma=1$; pam&$\mathbf{1}$&$\mathbf{0}$\tabularnewline
        ASW& 2&Rimle&$\gamma=1$;; kmeans&$\mathbf{1}$&$\mathbf{0}$\tabularnewline
        FW& 2&Rimle&$\gamma=100$;; kmeans&$0.98$&$-0.08$\tabularnewline
        CVLK& 3&Rimle&$\gamma=10$; InitClust&$0.85$&$-0.42$\tabularnewline
        CVQH& 3&Mclust& VEV&$0.78$&$-0.62$\tabularnewline
        CVQS& 3&Mclust& VEV&$0.78$&$-0.62$\tabularnewline
        BQH& 3&Rimle&$\gamma=10$;; kmeans&$0.86$&$-0.37$\tabularnewline
        BQS& 3&Rimle&$\gamma=10$;; kmeans&$0.86$&$-0.37$\tabularnewline
        \bottomrule
        \end{tabular}
    }\\

    \subfloat[][Olive dataset (3 classes)]{
        \begin{tabular}{lrllrr}
        \toprule
        \multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
        \midrule
        BEST ARI& 3&Emmix&mvt; $\text{ncov}=3$&$1$&$-0.03$\tabularnewline
        BEST VIC& 3&Emmix&mvt; $\text{ncov}=3$&$1$&$-0.03$\tabularnewline
        \midrule
        AIC&10&Emmix&mvt; $\text{ncov}=3$&$0.33$&$-1.74$\tabularnewline
        BIC& 6&Emmix&mvt; $\text{ncov}=3$&$0.52$&$-1.42$\tabularnewline
        ICL& 6&Emmix&mvt; $\text{ncov}=3$&$0.52$&$-1.42$\tabularnewline
        QH&10&Mclust& VVV&$0.29$&$-1.84$\tabularnewline
        QS&10&Mclust& VVV&$0.29$&$-1.84$\tabularnewline
        CH& 3&K-Means&&$0.32$&$-1.88$\tabularnewline
        ASW& 2&Emmix&mvt; $\text{ncov}=5$&$0.39$&$-1.28$\tabularnewline
        FW& 2&Emmix&mvt; $\text{ncov}=3$&$\mathbf{0.82}$&$\mathbf{-0.42}$\tabularnewline
        CVLK&10&Rimle&$\gamma=1000$; InitClust&$0.3$&$-1.81$\tabularnewline
        CVQH& 7&Emmix&mvt; $\text{ncov}=3$&$0.28$&$-2.04$\tabularnewline
        CVQS& 7&Emmix&mvt; $\text{ncov}=3$&$0.28$&$-2.04$\tabularnewline
        BQH& 8&Mclust& VVV&$0.49$&$-1.28$\tabularnewline
        BQS& 8&Mclust& VVV&$0.49$&$-1.28$\tabularnewline
        \bottomrule
        \end{tabular}
    }
    \subfloat[][Olive dataset (9 classes)]{
        \begin{tabular}{lrllrr}
        \toprule
        \multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{K}&\multicolumn{1}{c}{Algorithm}&\multicolumn{1}{c}{Configuration}&\multicolumn{1}{c}{ARI}&\multicolumn{1}{c}{VIC}\tabularnewline
        \midrule
        BEST ARI& 8&Mclust& EVE&$0.88$&$-0.65$\tabularnewline
        BEST VIC& 8&Mclust& EVE&$0.88$&$-0.65$\tabularnewline
        \midrule
        AIC&10&Emmix&mvt; $\text{ncov}=3$&$0.47$&$-1.77$\tabularnewline
        BIC& 6&Emmix&mvt; $\text{ncov}=3$&$0.76$&$-1.32$\tabularnewline
        ICL& 6&Emmix&mvt; $\text{ncov}=3$&$0.76$&$-1.32$\tabularnewline
        QH&10&Mclust& VVV&$0.54$&$-1.26$\tabularnewline
        QS&10&Mclust& VVV&$0.54$&$-1.26$\tabularnewline
        CH& 3&K-Means&&$0.42$&$-2.28$\tabularnewline
        ASW& 2&Emmix&mvt; $\text{ncov}=5$&$0.29$&$-2.28$\tabularnewline
        FW& 2&Emmix&mvt; $\text{ncov}=3$&$0.36$&$-1.84$\tabularnewline
        CVLK&10&Rimle&$\gamma=1000$; InitClust&$0.58$&$-1.18$\tabularnewline
        CVQH& 7&Emmix&mvt; $\text{ncov}=3$&$0.44$&$-1.96$\tabularnewline
        CVQS& 7&Emmix&mvt; $\text{ncov}=3$&$0.44$&$-1.96$\tabularnewline
        BQH& 8&Mclust& VVV&$\mathbf{0.86}$&$\mathbf{-0.74}$\tabularnewline
        BQS& 8&Mclust& VVV&$\mathbf{0.86}$&$\mathbf{-0.74}$\tabularnewline
        \bottomrule
        \end{tabular}
    }
\end{sidewaystable}


==> tables/simulated_tables.tex <==
\begin{table}
\tiny
\centering
\caption{Simulated datasets results}\label{tab:simulated_tables}
\subfloat[Pentagon5\label{tab:simulated_tables:pentagon5}]{
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{Mean ARI}&\multicolumn{1}{c}{Mean VIC}&\multicolumn{1}{c}{Med. ARI}&\multicolumn{1}{c}{Med. VIC}&\multicolumn{1}{c}{1st K}&\multicolumn{1}{c}{2nd K}\tabularnewline
\midrule
BEST ARI&$0.92 \pm (0.02)$&&$0.92$&&$5\;(0.83)$&$4\;(0.1)$\tabularnewline
BEST VIC&&$-0.36 \pm (0.07)$&&$-0.36$&$4\;(0.52)$&$5\;(0.34)$\tabularnewline
AIC&$0.82 \pm (0.11)$&$-0.66 \pm (0.31)$&$0.87$&$-0.57$&$5\;(0.59)$&$6\;(0.11)$\tabularnewline
BIC&$\mathbf{0.88 \pm (0.04)}$&$-0.43 \pm (0.09)$&$\mathbf{0.89}$&$\mathbf{-0.43}$&$5\;(0.45)$&$4\;(0.3)$\tabularnewline
ICL&$0.85 \pm (0.03)$&$\mathbf{-0.42 \pm (0.06)}$&$0.84$&$\mathbf{-0.43}$&$3\;(0.88)$&$4\;(0.08)$\tabularnewline
HS&$0.76 \pm (0.12)$&$-0.89 \pm (0.36)$&$0.80$&$-0.83$&$10\;(0.31)$&$7\;(0.16)$\tabularnewline
SS&$0.84 \pm (0.07)$&$-0.57 \pm (0.25)$&$0.86$&$-0.48$&$4\;(0.39)$&$3\;(0.16)$\tabularnewline
CH&$0.84 \pm (0.02)$&$-0.43 \pm (0.05)$&$0.84$&$-0.44$&$3\;(1)$&\tabularnewline
ASW&$0.84 \pm (0.03)$&$-0.43 \pm (0.06)$&$0.84$&$\mathbf{-0.43}$&$3\;(1)$&$4\;(0)$\tabularnewline
FW&$0.84 \pm (0.06)$&$-0.43 \pm (0.1)$&$0.84$&$\mathbf{-0.43}$&$3\;(0.99)$&$2\;(0.01)$\tabularnewline
CVLK&$0.73 \pm (0.13)$&$-0.85 \pm (0.33)$&$0.75$&$-0.82$&$6\;(0.32)$&$5\;(0.23)$\tabularnewline
CVHS&$0.82 \pm (0.09)$&$-0.58 \pm (0.25)$&$0.85$&$-0.50$&$4\;(0.42)$&$3\;(0.32)$\tabularnewline
CVSS&$0.84 \pm (0.05)$&$-0.48 \pm (0.13)$&$0.85$&$-0.45$&$3\;(0.61)$&$4\;(0.31)$\tabularnewline
BTHS&$0.85 \pm (0.03)$&$-0.43 \pm (0.06)$&$0.84$&$-0.44$&$3\;(0.9)$&$4\;(0.08)$\tabularnewline
BTSS&$0.84 \pm (0.03)$&$-0.43 \pm (0.06)$&$0.84$&$-0.44$&$3\;(0.98)$&$4\;(0.02)$\tabularnewline
\bottomrule
\end{tabular}
}

\vspace{1em}

\subfloat[Uniform\label{tab:simulated_tables:uniform}]{
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{Mean ARI}&\multicolumn{1}{c}{Mean VIC}&\multicolumn{1}{c}{Med. ARI}&\multicolumn{1}{c}{Med. VIC}&\multicolumn{1}{c}{1st K}&\multicolumn{1}{c}{2nd K}\tabularnewline
\midrule
BEST ARI&$1 \pm (0)$&&$1$&&$1\;(1)$&\tabularnewline
BEST VIC&&$0 \pm (0)$&&$0$&$1\;(1)$&\tabularnewline
AIC&$0 \pm (0)$&$-3.01 \pm (0.22)$&$0$&$-3.03$&$10\;(0.51)$&$9\;(0.27)$\tabularnewline
BIC&$0 \pm (0)$&$-1.94 \pm (0.4)$&$0$&$-1.98$&$4\;(0.65)$&$5\;(0.13)$\tabularnewline
ICL&$0.77 \pm (0.42)$&$-0.22 \pm (0.45)$&$\mathbf{1}$&$ 0.00$&$1\;(0.77)$&$2\;(0.18)$\tabularnewline
HS&$0 \pm (0)$&$-3.1 \pm (0.11)$&$0$&$-3.12$&$10\;(0.9)$&$9\;(0.08)$\tabularnewline
SS&$0.16 \pm (0.37)$&$-2.61 \pm (1.14)$&$0$&$-3.10$&$10\;(0.71)$&$1\;(0.16)$\tabularnewline
CH&$0 \pm (0)$&$-3.06 \pm (0.41)$&$0$&$-3.16$&$10\;(0.46)$&$9\;(0.38)$\tabularnewline
ASW&$0 \pm (0)$&$-2.1 \pm (0.37)$&$0$&$-1.99$&$4\;(0.74)$&$3\;(0.07)$\tabularnewline
FW&$0 \pm (0)$&$-2.38 \pm (0.59)$&$0$&$-1.99$&$4\;(0.64)$&$10\;(0.18)$\tabularnewline
CVLK&$0 \pm (0)$&$-2.84 \pm (0.28)$&$0$&$-2.84$&$8\;(0.3)$&$9\;(0.24)$\tabularnewline
CVHS&$0.06 \pm (0.24)$&$-2.3 \pm (0.81)$&$0$&$-2.55$&$7\;(0.22)$&$6\;(0.19)$\tabularnewline
CVSS&$0.85 \pm (0.35)$&$-0.25 \pm (0.73)$&$\mathbf{1}$&$ 0.00$&$1\;(0.85)$&$2\;(0.07)$\tabularnewline
BTHS&$0 \pm (0)$&$-3.14 \pm (0.31)$&$0$&$-3.21$&$10\;(0.82)$&$9\;(0.1)$\tabularnewline
BTSS&$\mathbf{0.96 \pm (0.19)}$&$\mathbf{-0.1 \pm (0.54)}$&$\mathbf{1}$&$ 0.00$&$1\;(0.96)$&$10\;(0.03)$\tabularnewline
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}
    \tiny
    \centering
    \ContinuedFloat
    \caption{}
\subfloat[Flower2\label{tab:simulated_tables:flower2}]{
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{Mean ARI}&\multicolumn{1}{c}{Mean VIC}&\multicolumn{1}{c}{Med. ARI}&\multicolumn{1}{c}{Med. VIC}&\multicolumn{1}{c}{1st K}&\multicolumn{1}{c}{2nd K}\tabularnewline
\midrule
BEST ARI&$0.68 \pm (0.06)$&&$0.69$&&$5\;(0.73)$&$6\;(0.11)$\tabularnewline
BEST VIC&&$-1.21 \pm (0.17)$&&$-1.21$&$5\;(0.77)$&$4\;(0.18)$\tabularnewline
AIC&$0.48 \pm (0.1)$&$-1.91 \pm (0.34)$&$0.48$&$-1.89$&$8\;(0.24)$&$9\;(0.22)$\tabularnewline
BIC&$0.32 \pm (0.1)$&$-1.88 \pm (0.22)$&$0.29$&$-1.92$&$2\;(0.58)$&$3\;(0.33)$\tabularnewline
ICL&$0.35 \pm (0.12)$&$-1.8 \pm (0.26)$&$0.30$&$-1.90$&$2\;(0.65)$&$3\;(0.2)$\tabularnewline
HS&$0.47 \pm (0.07)$&$-1.96 \pm (0.21)$&$0.47$&$-1.97$&$10\;(0.85)$&$9\;(0.13)$\tabularnewline
SS&$0.46 \pm (0.08)$&$-1.88 \pm (0.22)$&$0.46$&$-1.89$&$10\;(0.59)$&$9\;(0.21)$\tabularnewline
CH&$0.44 \pm (0.04)$&$-1.98 \pm (0.17)$&$0.44$&$-1.98$&$10\;(0.87)$&$9\;(0.08)$\tabularnewline
ASW&$0.45 \pm (0.17)$&$-1.58 \pm (0.29)$&$0.50$&$-1.50$&$5\;(0.85)$&$2\;(0.1)$\tabularnewline
FW&$0.45 \pm (0.1)$&$-1.6 \pm (0.21)$&$0.46$&$-1.60$&$5\;(0.86)$&$2\;(0.09)$\tabularnewline
CVLK&$0.49 \pm (0.11)$&$-1.8 \pm (0.27)$&$0.51$&$-1.79$&$7\;(0.43)$&$8\;(0.23)$\tabularnewline
CVHS&$0.47 \pm (0.13)$&$-1.73 \pm (0.27)$&$0.48$&$-1.73$&$6\;(0.27)$&$7\;(0.27)$\tabularnewline
CVSS&$0.43 \pm (0.14)$&$-1.74 \pm (0.27)$&$0.46$&$-1.80$&$5\;(0.23)$&$6\;(0.22)$\tabularnewline
BTHS&$\mathbf{0.53 \pm (0.09)}$&$\mathbf{-1.51 \pm (0.25)}$&$\mathbf{0.52}$&$\mathbf{-1.49}$&$5\;(0.74)$&$9\;(0.08)$\tabularnewline
BTSS&$0.46 \pm (0.11)$&$-1.58 \pm (0.24)$&$0.49$&$-1.52$&$5\;(0.72)$&$2\;(0.23)$\tabularnewline
\bottomrule
\end{tabular}
}

\vspace{1em}

\subfloat[T52D\label{tab:simulated_tables:t52d}]{
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{Mean ARI}&\multicolumn{1}{c}{Mean VIC}&\multicolumn{1}{c}{Med. ARI}&\multicolumn{1}{c}{Med. VIC}&\multicolumn{1}{c}{1st K}&\multicolumn{1}{c}{2nd K}\tabularnewline
\midrule
BEST ARI&$0.99 \pm (0.01)$&&$0.99$&&$5\;(0.99)$&$4\;(0.01)$\tabularnewline
BEST VIC&&$-0.06 \pm (0.05)$&&$-0.05$&$5\;(0.97)$&$4\;(0.01)$\tabularnewline
AIC&$0.84 \pm (0.13)$&$-0.5 \pm (0.32)$&$0.86$&$-0.48$&$6\;(0.21)$&$9\;(0.2)$\tabularnewline
BIC&$0.97 \pm (0.04)$&$-0.12 \pm (0.1)$&$0.98$&$-0.10$&$5\;(0.9)$&$6\;(0.09)$\tabularnewline
ICL&$0.98 \pm (0.01)$&$-0.11 \pm (0.08)$&$\mathbf{0.99}$&$-0.09$&$5\;(0.95)$&$4\;(0.04)$\tabularnewline
HS&$0.85 \pm (0.1)$&$-0.55 \pm (0.26)$&$0.86$&$-0.58$&$10\;(0.41)$&$9\;(0.19)$\tabularnewline
SS&$0.91 \pm (0.08)$&$-0.35 \pm (0.25)$&$0.93$&$-0.29$&$10\;(0.21)$&$5\;(0.2)$\tabularnewline
CH&$0.7 \pm (0.1)$&$-0.7 \pm (0.26)$&$0.68$&$-0.71$&$7\;(0.4)$&$6\;(0.31)$\tabularnewline
ASW&$0.92 \pm (0.15)$&$-0.26 \pm (0.32)$&$0.97$&$-0.16$&$5\;(0.86)$&$2\;(0.13)$\tabularnewline
FW&$0.59 \pm (0.18)$&$-0.93 \pm (0.36)$&$0.51$&$-1.08$&$2\;(0.81)$&$4\;(0.13)$\tabularnewline
CVLK&$0.84 \pm (0.13)$&$-0.44 \pm (0.27)$&$0.89$&$-0.34$&$6\;(0.41)$&$7\;(0.24)$\tabularnewline
CVHS&$0.9 \pm (0.11)$&$-0.32 \pm (0.23)$&$0.95$&$-0.26$&$4\;(0.43)$&$5\;(0.31)$\tabularnewline
CVSS&$0.93 \pm (0.08)$&$-0.27 \pm (0.19)$&$0.95$&$-0.24$&$4\;(0.54)$&$5\;(0.31)$\tabularnewline
BTHS&$\mathbf{0.99 \pm (0.01)}$&$\mathbf{-0.08 \pm (0.06)}$&$\mathbf{0.99}$&$\mathbf{-0.07}$&$5\;(0.98)$&$4\;(0.01)$\tabularnewline
BTSS&$\mathbf{0.99 \pm (0.01)}$&$\mathbf{-0.08 \pm (0.06)}$&$\mathbf{0.99}$&$\mathbf{-0.07}$&$5\;(0.98)$&$4\;(0.01)$\tabularnewline
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}
    \tiny
    \centering
    \ContinuedFloat
    \caption{}
\subfloat[T510D\label{tab:simulated_tables:t510d}]{
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Criterion}&\multicolumn{1}{c}{Mean ARI}&\multicolumn{1}{c}{Mean VIC}&\multicolumn{1}{c}{Med. ARI}&\multicolumn{1}{c}{Med. VIC}&\multicolumn{1}{c}{1st K}&\multicolumn{1}{c}{2nd K}\tabularnewline
\midrule
BEST ARI&$0.99 \pm (0.01)$&&$0.99$&&$5\;(0.99)$&$4\;(0.01)$\tabularnewline
BEST VIC&&$-0.09 \pm (0.06)$&&$-0.09$&$5\;(0.99)$&$4\;(0.01)$\tabularnewline
AIC&$0.7 \pm (0.13)$&$-1.06 \pm (0.43)$&$0.68$&$-1.03$&$9\;(0.24)$&$10\;(0.24)$\tabularnewline
BIC&$0.86 \pm (0.1)$&$-0.35 \pm (0.18)$&$0.82$&$-0.41$&$6\;(0.5)$&$5\;(0.49)$\tabularnewline
ICL&$\mathbf{0.94 \pm (0.08)}$&$-0.23 \pm (0.15)$&$0.97$&$-0.19$&$5\;(0.83)$&$6\;(0.16)$\tabularnewline
HS&$0.55 \pm (0.08)$&$-1.23 \pm (0.32)$&$0.53$&$-1.20$&$10\;(0.98)$&$9\;(0.02)$\tabularnewline
SS&$0.55 \pm (0.07)$&$-1.2 \pm (0.23)$&$0.53$&$-1.19$&$10\;(0.98)$&$9\;(0.02)$\tabularnewline
CH&$0.51 \pm (0.03)$&$-1.1 \pm (0.05)$&$0.50$&$-1.11$&$2\;(1)$&\tabularnewline
ASW&$0.51 \pm (0.03)$&$-1.1 \pm (0.05)$&$0.51$&$-1.11$&$2\;(1)$&\tabularnewline
FW&$0.53 \pm (0.11)$&$-1.05 \pm (0.21)$&$0.50$&$-1.10$&$2\;(0.94)$&$5\;(0.04)$\tabularnewline
CVLK&$0.74 \pm (0.13)$&$-0.75 \pm (0.43)$&$0.74$&$-0.67$&$6\;(0.45)$&$7\;(0.38)$\tabularnewline
CVHS&$0.79 \pm (0.13)$&$-0.62 \pm (0.33)$&$0.79$&$-0.58$&$5\;(0.36)$&$6\;(0.35)$\tabularnewline
CVSS&$0.8 \pm (0.13)$&$-0.61 \pm (0.34)$&$0.79$&$-0.58$&$5\;(0.38)$&$6\;(0.29)$\tabularnewline
BTHS&$0.91 \pm (0.12)$&$-0.28 \pm (0.26)$&$0.97$&$-0.19$&$5\;(0.69)$&$6\;(0.19)$\tabularnewline
BTSS&$\mathbf{0.94 \pm (0.09)}$&$\mathbf{-0.2 \pm (0.18)}$&$\mathbf{0.98}$&$\mathbf{-0.15}$&$5\;(0.85)$&$6\;(0.1)$\tabularnewline
\bottomrule
\end{tabular}
}
\end{table}

